Signature Isolation Forest

Functional Isolation Forest (FIF) is a recent state-of-the-art Anomaly Detection (AD) algorithm designed for functional data. It relies on a tree partition procedure where an abnormality score is computed by projecting each curve observation on a drawn dictionary through a linear inner product. Such linear inner product and the dictionary are a priori choices that highly influence the algorithm's performances and might lead to unreliable results, particularly with complex datasets. This work addresses these challenges by introducing \textit{Signature Isolation Forest}, a novel AD algorithm class leveraging the rough path theory's signature transform. Our objective is to remove the constraints imposed by FIF through the proposition of two algorithms which specifically target the linearity of the FIF inner product and the choice of the dictionary. We provide several numerical experiments, including a real-world applications benchmark showing the relevance of our methods.

==> sif <==
\begin{thebibliography}{}

\bibitem[Breunig et~al., 2000]{Breunig}
Breunig, M., Kriegel, H.-P., Ng, R., and Sander, J. (2000).
\newblock {LOF}: Identifying density-based local outliers.
\newblock In {\em Proceedings of the 2000 ACM SIGMOD International Conference on Management of Data}, volume~29, pages 93--104. ACM.

\bibitem[Chandola et~al., 2009]{Chandola}
Chandola, V., Banerjee, A., and Kumar, V. (2009).
\newblock Anomaly detection: A survey.
\newblock {\em ACM Computing Surveys (CSUR)}, 41(3):15:1--15:58.

\bibitem[Chen, 1958]{chen1958integration}
Chen, K.-T. (1958).
\newblock Integration of paths--a faithful representation of paths by noncommutative formal power series.
\newblock {\em Transactions of the American Mathematical Society}, 89(2):395--407.

\bibitem[Chen et~al., 2015]{UCRArchive}
Chen, Y., Keogh, E., Hu, B., Begum, N., Bagnall, A., Mueen, A., and Batista, G. (2015).
\newblock The {UCR} time series classification archive.

\bibitem[Chevyrev and Kormilitzin, 2016]{chevyrev2016primer}
Chevyrev, I. and Kormilitzin, A. (2016).
\newblock A primer on the signature method in machine learning.
\newblock {\em arXiv preprint arXiv:1603.03788}.

\bibitem[Chevyrev and Oberhauser, 2022]{chevyrev2022signature}
Chevyrev, I. and Oberhauser, H. (2022).
\newblock Signature moments to characterize laws of stochastic processes.
\newblock {\em The Journal of Machine Learning Research}, 23(1):7928--7969.

\bibitem[Claeskens et~al., 2014]{claeskens2014multivariate}
Claeskens, G., Hubert, M., Slaets, L., and Vakili, K. (2014).
\newblock Multivariate functional halfspace depth.
\newblock {\em Journal of the American Statistical Association}, 109(505):411--423.

\bibitem[Cuevas et~al., 2007]{cuevas}
Cuevas, A., Febrero, M., and Fraiman, R. (2007).
\newblock Robust estimation and classification for functional data via projection-based depth notions.
\newblock {\em Computational Statistics}, 22(3):481--496.

\bibitem[Dauxois et~al., 1982]{dauxois1982asymptotic}
Dauxois, J., Pousse, A., and Romain, Y. (1982).
\newblock Asymptotic theory for the principal component analysis of a vector random function: some applications to statistical inference.
\newblock {\em Journal of multivariate analysis}, 12(1):136--154.

\bibitem[Fermanian, 2021]{fermanian2021embedding}
Fermanian, A. (2021).
\newblock Embedding and learning with signatures.
\newblock {\em Computational Statistics \& Data Analysis}, 157:107148.

\bibitem[Ferraty, 2006]{ferraty2006nonparametric}
Ferraty, F. (2006).
\newblock {\em Nonparametric functional data analysis}.
\newblock Springer.

\bibitem[Fraiman and Muniz, 2001]{fraiman2001trimmed}
Fraiman, R. and Muniz, G. (2001).
\newblock Trimmed means for functional data.
\newblock {\em Test}, 10:419--440.

\bibitem[Friz and Victoir, 2010]{friz2010multidimensional}
Friz, P.~K. and Victoir, N.~B. (2010).
\newblock {\em Multidimensional stochastic processes as rough paths: theory and applications}, volume 120.
\newblock Cambridge University Press.

\bibitem[Gijbels and Nagy, 2017]{nagyfunctional}
Gijbels, I. and Nagy, S. (2017).
\newblock {On a General Definition of Depth for Functional Data}.
\newblock {\em Statistical Science}, 32(4):630 -- 639.

\bibitem[Hubert et~al., 2015]{hubert2015multivariate}
Hubert, M., Rousseeuw, P.~J., and Segaert, P. (2015).
\newblock Multivariate functional outlier detection.
\newblock {\em Statistical Methods \& Applications}, 24(2):177--202.

\bibitem[Kir{\'a}ly and Oberhauser, 2019]{kiraly2019kernels}
Kir{\'a}ly, F.~J. and Oberhauser, H. (2019).
\newblock Kernels for sequentially ordered data.
\newblock {\em Journal of Machine Learning Research}, 20.

\bibitem[Lee and Oberhauser, 2023]{lee2023signature}
Lee, D. and Oberhauser, H. (2023).
\newblock The signature kernel.
\newblock {\em arXiv preprint arXiv:2305.04625}.

\bibitem[Liu et~al., 2008]{liu2008isolation}
Liu, F.~T., Ting, K.~M., and Zhou, Z.-H. (2008).
\newblock Isolation forest.
\newblock In {\em 2008 eighth ieee international conference on data mining}, pages 413--422. IEEE.

\bibitem[L{\'o}pez-Pintado and Romo, 2009]{lopez2009concept}
L{\'o}pez-Pintado, S. and Romo, J. (2009).
\newblock On the concept of depth for functional data.
\newblock {\em Journal of the American statistical Association}, pages 718--734.

\bibitem[L{\'o}pez-Pintado and Romo, 2011]{lopez2011half}
L{\'o}pez-Pintado, S. and Romo, J. (2011).
\newblock A half-region depth for functional data.
\newblock {\em Computational Statistics \& Data Analysis}, 55(4):1679--1695.

\bibitem[Lyons and McLeod, 2022]{lyons2022signature}
Lyons, T. and McLeod, A.~D. (2022).
\newblock Signature methods in machine learning.
\newblock {\em arXiv preprint arXiv:2206.14674}.

\bibitem[Lyons et~al., 2007]{lyons2007differential}
Lyons, T.~J., Caruana, M., and L{\'e}vy, T. (2007).
\newblock {\em Differential equations driven by rough paths}.
\newblock Springer.

\bibitem[Morrill et~al., 2019]{morrill2019signature}
Morrill, J., Kormilitzin, A., Nevado-Holgado, A., Swaminathan, S., Howison, S., and Lyons, T. (2019).
\newblock The signature-based model for early detection of sepsis from electronic health records in the intensive care unit.
\newblock In {\em 2019 Computing in Cardiology (CinC)}, pages Page--1. IEEE.

\bibitem[Nieto-Reyes and Battey, 2016]{nieto2016}
Nieto-Reyes, A. and Battey, H. (2016).
\newblock {A Topologically Valid Definition of Depth for Functional Data}.
\newblock {\em Statistical Science}, 31(1):61 -- 79.

\bibitem[Polonik, 1997]{polonik1997minimum}
Polonik, W. (1997).
\newblock Minimum volume sets and generalized quantile processes.
\newblock {\em Stochastic processes and their applications}, 69(1):1--24.

\bibitem[Ramsay and Silverman, 2005]{ramsay2005fitting}
Ramsay, J.~O. and Silverman, B.~W. (2005).
\newblock {\em Fitting differential equations to functional data: Principal differential analysis}.
\newblock Springer.

\bibitem[Reutenauer, 2003]{reutenauer2003free}
Reutenauer, C. (2003).
\newblock Free lie algebras.
\newblock In {\em Handbook of algebra}, volume~3, pages 887--903. Elsevier.

\bibitem[Rossi and Villa, 2006]{rossi2006support}
Rossi, F. and Villa, N. (2006).
\newblock Support vector machine for functional data classification.
\newblock {\em Neurocomputing}, 69(7-9):730--742.

\bibitem[Rousseeuw and Driessen, 1999]{rousseeuw1999fast}
Rousseeuw, P.~J. and Driessen, K.~V. (1999).
\newblock A fast algorithm for the minimum covariance determinant estimator.
\newblock {\em Technometrics}, 41(3):212--223.

\bibitem[Salvi et~al., 2021]{salvi2021signature}
Salvi, C., Cass, T., Foster, J., Lyons, T., and Yang, W. (2021).
\newblock The signature kernel is the solution of a goursat pde.
\newblock {\em SIAM Journal on Mathematics of Data Science}, 3(3):873--899.

\bibitem[Sch\"olkopf et~al., 2001]{SPSSW01}
Sch\"olkopf, B., Platt, J., Shawe-Taylor, J., Smola, A., and Williamson, R. (2001).
\newblock Estimating the support of a high-dimensional distribution.
\newblock {\em Neural Computation}, 13(7):1443--1471.

\bibitem[Sch{\"o}lkopf et~al., 2001]{scholkopf2001estimating}
Sch{\"o}lkopf, B., Platt, J.~C., Shawe-Taylor, J., Smola, A.~J., and Williamson, R.~C. (2001).
\newblock Estimating the support of a high-dimensional distribution.
\newblock {\em Neural computation}, 13(7):1443--1471.

\bibitem[Shang, 2014]{shang2014survey}
Shang, H.~L. (2014).
\newblock A survey of functional principal component analysis.
\newblock {\em AStA Advances in Statistical Analysis}, 98:121--142.

\bibitem[Staerman, 2022]{staerman2022functional}
Staerman, G. (2022).
\newblock {\em Functional anomaly detection and robust estimation}.
\newblock PhD thesis, Institut polytechnique de Paris.

\bibitem[Staerman et~al., 2023]{staerman2023}
Staerman, G., Adjakossa, E., Mozharovskyi, P., Hofer, V., Sen~Gupta, J., and Cl{\'e}men{\c c}on, S. (2023).
\newblock Functional anomaly detection: a benchmark study.
\newblock {\em International Journal of Data Science and Analytics}, 16(1):101--117.

\bibitem[Staerman et~al., 2020]{staerman2020area}
Staerman, G., Mozharovskyi, P., Cl{\'e}men, S., et~al. (2020).
\newblock The area of the convex hull of sampled curves: a robust functional statistical depth measure.
\newblock In {\em International Conference on Artificial Intelligence and Statistics}, pages 570--579. PMLR.

\bibitem[Staerman et~al., 2019]{staerman2019functional}
Staerman, G., Mozharovskyi, P., Cl{\'e}men{\c{c}}on, S., and d’Alch{\'e} Buc, F. (2019).
\newblock Functional isolation forest.
\newblock In {\em Asian Conference on Machine Learning}, pages 332--347. PMLR.

\bibitem[Wang et~al., 2016]{wang2016functional}
Wang, J.-L., Chiou, J.-M., and M{\"u}ller, H.-G. (2016).
\newblock Functional data analysis.
\newblock {\em Annual Review of Statistics and its application}, 3:257--295.

\bibitem[Wilson-Nunn et~al., 2018]{wilson2018path}
Wilson-Nunn, D., Lyons, T., Papavasiliou, A., and Ni, H. (2018).
\newblock A path signature approach to online arabic handwriting recognition.
\newblock In {\em 2018 IEEE 2nd International Workshop on Arabic and Derived Script Analysis and Recognition (ASAR)}, pages 135--139. IEEE.

\bibitem[Yang et~al., 2016a]{yang2016deepwriterid}
Yang, W., Jin, L., and Liu, M. (2016a).
\newblock Deepwriterid: An end-to-end online text-independent writer identification system.
\newblock {\em IEEE Intelligent Systems}, 31(2):45--53.

\bibitem[Yang et~al., 2016b]{yang2016dropsample}
Yang, W., Jin, L., Tao, D., Xie, Z., and Feng, Z. (2016b).
\newblock Dropsample: A new training method to enhance deep convolutional neural networks for large-scale unconstrained handwritten chinese character recognition.
\newblock {\em Pattern Recognition}, 58:190--203.

\end{thebibliography}

